Preventing Verbatim Memorization in Language Models Gives a False Sense of Privacy

Studying data memorization in neural language models helps us understand the risks (e.g., to privacy or copyright) associated with models regurgitating training data and aids in the development of countermeasures. Many prior works -- and some recently deployed defenses -- focus on "verbatim memorization", defined as a model generation that exactly matches a substring from the training set. We argue that verbatim memorization definitions are too restrictive and fail to capture more subtle forms of memorization. Specifically, we design and implement an efficient defense that perfectly prevents all verbatim memorization. And yet, we demonstrate that this "perfect" filter does not prevent the leakage of training data. Indeed, it is easily circumvented by plausible and minimally modified "style-transfer" prompts -- and in some cases even the non-modified original prompts -- to extract memorized information. We conclude by discussing potential alternative definitions and why defining memorization is a difficult yet crucial open question for neural language models.

==> figures/bloom_filter_stats.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{\textbf{Something useful about this table.} Bloom filter hit statistics.}
    \label{tab:my_label}
\end{table}

==> tables/approx_mem_at_threshold.tex <==
\begin{table*}
    \centering
    \small
    \begin{tabular}{p{2.5in}|p{2.5in}|r}
    \toprule
        \textbf{True Continuation} & \textbf{LM Generation} & BLEU \\
        \midrule
         about a deeper bond with the product. Nostalgia. It’s delicate, but potent. Sweetheart.\textbackslash n\textbackslash nTeddy told me that in Greek, “nostalgia” literally means “the pain from an old wound”. It’s a twinge in your heart far more & about a deeper bond with a product. Nostalgia. It's delicate, but potent. Teddy told me that in Greek, nostalgia literally means the pain from an old wound. It's a twinge in your heart, far more powerful than memory alone. This	& 0.79\\
         \midrule
         And I'll show you\textbackslash nYou want the moves like jagger\textbackslash nI got the moves like jagger\textbackslash nI got the mooooooves like jagger\textbackslash nI don't even try to control you\textbackslash nLook into my eyes and I'll own you\textbackslash nYou with the moves	&
         And I'll show you\textbackslash nAll the moves like Jagger\textbackslash nI've got the moves like Jagger\textbackslash nI've got the moves like Jagger\textbackslash nI don't need to try to control you\textbackslash nLook into my eyes and I'll own you\textbackslash nWith the	& 0.79 \\
         \midrule
         Purpose\textbackslash n\textbackslash nThe laws of most jurisdictions throughout the world automatically confer\textbackslash nexclusive Copyright and Related Rights (defined below) upon the creator\textbackslash nand subsequent owner(s) (each and all, an "owner") of an original work of\textbackslash nauthorship and/or a database &
         Purpose\textbackslash n\textbackslash n The laws of most jurisdictions throughout the world automatically confer\textbackslash n exclusive Copyright and Related Rights (defined below) upon the creator\textbackslash n and subsequent owner(s) of an original work of authorship (the "Work").\textbackslash n Certain jurisdictions do not recognize a	& 0.76 \\
    \bottomrule
    \end{tabular}
    \caption{Examples of model generations with BLEU score close to 0.75, the threshold we used to declare that approximate memorization had occurred.}
    \label{tab:approx_mem_at_threshold}
\end{table*}
